MSSM Effects in Top-antitop Production at the LHC

We report on a calculation of the effects of supersymmetry on the cross-section for top-antitop production at LHC. A numerical study is carried out for the ten benchmarks of the Snowmass accord. It is found that the higher order effects involving supersymmetric particles in internal loops can be as high as 6%, both for the cross-section and the (parity even) helicity asymmetry, for one particular benchmark. For other benchmarks smaller but nonetheless observable corrections are found.

==> Makefile <==
MF=Makefile

MAIN=ttbarmssm
DVI=$(MAIN).dvi
PS=$(MAIN).ps
TAR=$(MAIN).tar.gz
PKG=$(MAIN)-pkg.tar.gz

TEX=\
paper.cls \
base.sty \
lang.sty \
fmslash.sty \
$(MAIN).bbl \
$(MAIN).tex \
title.tex \
intro.tex \
hel_mat_elem.tex \
prototypes.tex \
results.tex \
summary.tex 

ASY=\
$(MAIN).asy \
hel-diagrams.asy \
pro-diagrams.asy \
pro-selfenergies.asy

EPS=\
al.mtt.eps \
al.pt.eps \
pv.mtt.eps \
pv.pt.eps \
tot.mtt.eps \
tot.pt.eps \
tree.al.mtt.eps \
tree.al.pt.eps \
tree.tot.mtt.eps \
tree.tot.pt.eps \
llcomp.set5.gg.eps \
llcomp.set5.uu.eps \
llcomp.set5.dd.eps

ALLSRC=$(TEX) $(ASY) $(EPS) $(MF)

PIC_HEL_DIAGRAMS=\
hel-tree_slbl.eps \
hel-tree_s.eps hel-tree_s.tex \
hel-tree_t.eps hel-tree_t.tex \
hel-tree_u.eps hel-tree_u.tex \
hel-box.eps \
hel-xbox.eps

PIC_PRO_SELFENERGIES=\
pro-seF-SF.eps pro-seF-SF.tex \
pro-seF-VF.eps pro-seF-VF.tex \
pro-seG-FF.eps pro-seG-FF.tex \
pro-seG-SS.eps pro-seG-SS.tex \
pro-seG-S.eps pro-seG-S.tex

PIC_PRO_DIAGRAMS=\
pro-qqbar-sV-tree.eps \
pro-gg-sG-tree.eps \
pro-gg-tF-tree.eps \
pro-qqbar-sG-xseq-1.eps pro-qqbar-sG-xseq-1.tex \
pro-qqbar-sG-xseq-2.eps pro-qqbar-sG-xseq-2.tex \
pro-qqbar-sG-xset-1.eps pro-qqbar-sG-xset-1.tex \
pro-qqbar-sG-xset-2.eps pro-qqbar-sG-xset-2.tex \
pro-gg-sG-xseg-1.eps pro-gg-sG-xseg-1.tex \
pro-gg-sG-xseg-2.eps pro-gg-sG-xseg-2.tex \
pro-gg-sG-xset-1.eps pro-gg-sG-xset-1.tex \
pro-gg-sG-xset-2.eps pro-gg-sG-xset-2.tex \
pro-qqbar-sG-ise.eps \
pro-gg-sG-ise.eps \
pro-gg-tF-xseg-1.eps pro-gg-tF-xseg-1.tex \
pro-gg-tF-xseg-2.eps pro-gg-tF-xseg-2.tex \
pro-gg-tF-xset-1.eps pro-gg-tF-xset-1.tex \
pro-gg-tF-xset-2.eps pro-gg-tF-xset-2.tex \
pro-gg-tF-ise.eps \
pro-qqbar-sG-vertSq.eps \
pro-qqbar-sG-vertSt.eps \
pro-qqbar-sG-vertVq.eps \
pro-qqbar-sG-vertVt.eps \
pro-qqbar-sG-vertSSq.eps \
pro-qqbar-sG-vertSSt.eps \
pro-gg-sG-vertSt.eps \
pro-gg-sG-vertVt.eps \
pro-gg-sG-vertSSt.eps \
pro-gg-sZ-vertFg-ccw.eps pro-gg-sZ-vertFg-ccw.tex \
pro-gg-sZ-vertFg-cw.eps pro-gg-sZ-vertFg-cw.tex \
pro-gg-sG-vertFg-ccw.eps pro-gg-sG-vertFg-ccw.tex \
pro-gg-sG-vertFg-cw.eps pro-gg-sG-vertFg-cw.tex \
pro-gg-sG-vertSg-ccw.eps pro-gg-sG-vertSg-ccw.tex \
pro-gg-sG-vertSg-cw.eps pro-gg-sG-vertSg-cw.tex \
pro-gg-sS-vertFg-ccw.eps pro-gg-sS-vertFg-ccw.tex \
pro-gg-sS-vertFg-cw.eps pro-gg-sS-vertFg-cw.tex \
pro-gg-sS-vertSg-ccw.eps pro-gg-sS-vertSg-ccw.tex \
pro-gg-sS-vertSg-cw.eps pro-gg-sS-vertSg-cw.tex \
pro-gg-sS-vertSSg.eps \
pro-gg-tF-vertS1.eps \
pro-gg-tF-vertS2.eps \
pro-gg-tF-vertSS1.eps \
pro-gg-tF-vertSS2.eps \
pro-gg-tF-vertV1.eps \
pro-gg-tF-vertV2.eps \
pro-qqbar-boxSS.eps \
pro-qqbar-fboxSS.eps pro-qqbar-fboxSS.tex \
pro-qqbar-fboxSS-cr.eps pro-qqbar-fboxSS-cr.tex \
pro-qqbar-fboxSS-maj.eps pro-qqbar-fboxSS-maj.tex \
pro-qqbar-fboxSSx.eps pro-qqbar-fboxSSx.tex \
pro-qqbar-fboxSSx-cr.eps pro-qqbar-fboxSSx-cr.tex \
pro-qqbar-fboxSSx-maj.eps pro-qqbar-fboxSSx-maj.tex \
pro-qqbar-boxVV.eps \
pro-qqbar-boxVVx.eps \
pro-gg-boxFS.eps \
pro-gg-boxFV.eps \
pro-gg-boxSF.eps \
pro-gg-boxSFx.eps



PIC=\
$(PIC_HEL_DIAGRAMS) \
$(PIC_PRO_SELFENERGIES) \
$(PIC_PRO_DIAGRAMS)


all: $(PS)

.PHONY: backup
backup: $(TAR)

.PHONY: package
package: $(PKG)

$(DVI): $(TEX) $(PIC) $(EPS) $(MF)
	latex $(MAIN) && latex $(MAIN)

$(PS): $(DVI)
	dvips -o $(PS) $(DVI)

$(PIC_HEL_DIAGRAMS): hel-diagrams.asy $(MAIN).asy
	asy hel-diagrams.asy

$(PIC_PRO_SELFENERGIES): pro-selfenergies.asy ttbarmssm.asy
	asy pro-selfenergies.asy

$(PIC_PRO_DIAGRAMS): pro-diagrams.asy ttbarmssm.asy
	asy pro-diagrams.asy

$(TAR): $(ALLSRC)
	tar zcvf $(TAR) $(ALLSRC)

$(PKG): $(ALLSRC) $(PIC)
	tar zcvf $(PKG) $(ALLSRC) $(PIC)

.PHONY: clean
clean:
	rm -rf $(DVI) $(PS) $(PIC)


==> pro-gg-sZ-vertFg-ccw.tex <==
\raisebox{-69.682bp}{\includegraphics{pro-gg-sZ-vertFg-ccw}}

==> pro-gg-sZ-vertFg-cw.tex <==
\raisebox{-69.682bp}{\includegraphics{pro-gg-sZ-vertFg-cw}}

==> pro-qqbar-fboxSS-cr.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSS-cr}}

==> pro-qqbar-fboxSS-maj.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSS-maj}}

==> pro-qqbar-fboxSS.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSS}}

==> pro-qqbar-fboxSSx-cr.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSSx-cr}}

==> pro-qqbar-fboxSSx-maj.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSSx-maj}}

==> pro-qqbar-fboxSSx.tex <==
\raisebox{-56.5222bp}{\includegraphics{pro-qqbar-fboxSSx}}

==> pro-seF-VF.tex <==
\raisebox{-17.2591bp}{\includegraphics{pro-seF-VF}}
